MMFakeBench: A Mixed-Source Multimodal Misinformation Detection Benchmark for LVLMs

Current multimodal misinformation detection (MMD) methods often assume a single source and type of forgery for each sample, which is insufficient for real-world scenarios where multiple forgery sources coexist. The lack of a benchmark for mixed-source misinformation has hindered progress in this field. To address this, we introduce MMFakeBench, the first comprehensive benchmark for mixed-source MMD. MMFakeBench includes 3 critical sources: textual veracity distortion, visual veracity distortion, and cross-modal consistency distortion, along with 12 sub-categories of misinformation forgery types. We further conduct an extensive evaluation of 6 prevalent detection methods and 15 Large Vision-Language Models (LVLMs) on MMFakeBench under a zero-shot setting. The results indicate that current methods struggle under this challenging and realistic mixed-source MMD setting. Additionally, we propose MMD-Agent, a novel approach to integrate the reasoning, action, and tool-use capabilities of LVLM agents, significantly enhancing accuracy and generalization. We believe this study will catalyze future research into more realistic mixed-source multimodal misinformation and provide a fair evaluation of misinformation detection methods.

==> table/table4.tex <==


\begin{table*}[!t]
  \centering
%   \scriptsize
  \caption{Ablation studies on hierarchical decomposition and rationales $\mathcal{R} _t$ of each sub-task $t$. TVD denotes textual veracity distortion. VVD denotes visual veracity distortion. CCD denotes cross-modal consistency distortion.}
  \resizebox{\textwidth}{!}{%
\tablestyle{8pt}{1.4}
    \begin{tabular}{ccccccccc}
\hline
\textbf{Hieracical}  & \textbf{\begin{tabular}[c]{@{}c@{}}$\mathcal{R} _1$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\mathcal{R} _2$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\mathcal{R} _3$\end{tabular}} & \textbf{Original} & \textbf{\begin{tabular}[c]{@{}c@{}}TVD\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}VVD\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}CCD\end{tabular}} & \textbf{Overall} \\ \hline
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}                                                   & \multicolumn{1}{l}{}                                                   & \multicolumn{1}{l}{}                                                   & 58.5              & 5.8                                                                             & 0.0                                                                            & 38.6                                                                                   & 25.7             \\
\CheckmarkBold                 &                                                                        &                                                                        &                                                                        & 45.8              & 16.5 (\textcolor{gray}{$\uparrow$10.7})                                                                       & 32.5 (\textcolor{gray}{$\uparrow$32.5})                                                                      & 49.0 (\textcolor{gray}{$\uparrow$10.4})                                                                              & 36.0             \\
\CheckmarkBold                 & \CheckmarkBold                                                                   &                                                                        &                                                                        & 46.4              & 37.6 (\textcolor{gray}{$\uparrow$21.1})                                                                       & 32.8                                                                           & 47.2                                                                                   & 41.0             \\
\CheckmarkBold                 & \CheckmarkBold                                                                   & \CheckmarkBold                                                                   &                                                                        & 46.8              & 37.6                                                                            & 61.7 (\textcolor{gray}{$\uparrow$28.9})                                                                      & 48.6                                                                                   & 48.7             \\
\CheckmarkBold                 & \CheckmarkBold                                                                   & \CheckmarkBold                                                                   & \CheckmarkBold                                                                   & 51.1 (\textcolor{gray}{$\uparrow$4.3})          & 37.6                                                                            & 61.7                                                                           & 49.2 (\textcolor{gray}{$\uparrow$0.6})                                                                               & 49.9             \\ \hline
\end{tabular}
    }
    \vspace{-1.0em}
  \label{aba_pipeline}%
\end{table*}%
